ARLO: A Framework for Automated Reinforcement Learning

Automated Reinforcement Learning (AutoRL) is a relatively new area of research that is gaining increasing attention. The objective of AutoRL consists in easing the employment of Reinforcement Learning (RL) techniques for the broader public by alleviating some of its main challenges, including data collection, algorithm selection, and hyper-parameter tuning. In this work, we propose a general and flexible framework, namely ARLO: Automated Reinforcement Learning Optimizer, to construct automated pipelines for AutoRL. Based on this, we propose a pipeline for offline and one for online RL, discussing the components, interaction, and highlighting the difference between the two settings. Furthermore, we provide a Python implementation of such pipelines, released as an open-source library. Our implementation has been tested on an illustrative LQG domain and on classic MuJoCo environments, showing the ability to reach competitive performances requiring limited human intervention. We also showcase the full pipeline on a realistic dam environment, automatically performing the feature selection and the model generation tasks.

==> chapters/08_checklist.tex <==
\section{Reproducibility Checklist}
% The reproducibility checklist is a combination of the NeurIPS '21 checklist https://neurips.cc/Conferences/2021/PaperInformation/PaperChecklist and the NAS checklist https://www.automl.org/wp-content/uploads/NAS/NAS_checklist.pdf
% For each question, change the default \answerTODO{} to either:
%     \answerYes{[justification]},
%     \answerNo{[justification]},
%     \answerNA{[justification]}.
% *You must include a brief justification to your answer,* either by
% referencing the appropriate section of your paper or providing a brief inline
% description.  For example:
% - Did you include the license of the code and datasets?
%   \answerYes{See Section~\ref{sec:code}.}
% - Did you include all the code for running experiments?
%   \answerNo{We include the code we wrote, but it depends on proprietary
%   libraries for executing on a compute cluster and as such will not be
%   runnable without modifications. We also include a runnable sequential
%   version of the code that we also report experiments in the paper with.}
% - Did you include the license of the datasets?
%   \answerNA{Our experiments were conducted on publicly available datasets and we did not introduce new datasets.}
% Please note that if you answer a question with \answerNo{}, we expect that you compensate for it (e.g., if you cannot provide the full evaluation code, you should at least provide code for a minimal reproduction of the main insights of your paper). Please do not modify the questions and only use the provided macros for your answers. Note that this section does not count towards the page limit. 

\begin{enumerate}
\item For all authors\dots
  %
  \begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately
    reflect the paper's contributions and scope?
    %
    \answerYes{}
    %
  \item Did you describe the limitations of your work?
    %
    \answerYes{See Section \ref{sec:intro} and Section \ref{sec:conclusions}.}
    %
  \item Did you discuss any potential negative societal impacts of your work?
    %
    \answerYes{See Section \ref{sec:intro} and Section \ref{sec:conclusions}.}
    %
  \item Have you read the ethics review guidelines and ensured that your paper
    conforms to them?
    %
    \answerYes{}
    %
  \end{enumerate}
  %
\item If you are including theoretical results\dots
  %
  \begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    %
    \answerNA{}
    %
  \item Did you include complete proofs of all theoretical results?
    %
    \answerNA{}
    %
  \end{enumerate}
  %
\item If you ran experiments\dots
  %
  \begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the
    main experimental results, including all requirements (e.g.,
    \texttt{requirements.txt} with explicit version), an instructive
    \texttt{README} with installation, and execution commands (either in the
    supplemental material or as a \textsc{url})?
    %
    \answerYes{In the repository linked in the footnote on the second page and in Section \ref{sec:experiments}.}
    %
  \item Did you include the raw results of running the given instructions on the
    given code and data?
    %
    \answerNo{Unfortunately, adding all the data to the repository was not a viable option since the overall code+data would have been more than $30$ GB. Instead, we opt to include the code to generate the synthetically generated data and we added a reference to the real-world ones.}
    %
  \item Did you include scripts and commands that can be used to generate the
    figures and tables in your paper based on the raw results of the code, data,
    and instructions given?
    %
    \answerYes{In the repository linked in the footnote on the second page and in the Section \ref{sec:experiments}.}
    %
  \item Did you ensure sufficient code quality such that your code can be safely
    executed and the code is properly documented?
    %
    \answerYes{The documentation can be downloaded from the repository, linked in the footnote on the second page and in the Section \ref{sec:experiments}.}
    %
  \item Did you specify all the training details (e.g., data splits,
    pre-processing, search spaces, fixed hyperparameter settings, and how they
    were chosen)?
    %
    \answerYes{We specified that in the Supplementary Material.}
    %
  \item Did you ensure that you compared different methods (including your own)
    exactly on the same benchmarks, including the same datasets, search space,
    code for training and hyperparameters for that code?
    %
    \answerYes{We used the implementation of the proposed framework to run the experiments.}
    %
  \item Did you run ablation studies to assess the impact of different
    components of your approach?
    %
    \answerYes{Different experiments are meant to understand the capabilities of the different stages of the pipeline we defined.}
    %
  \item Did you use the same evaluation protocol for the methods being compared?
    %
    \answerYes{For a given experiment the evaluation protocol used was the same, as explained in the Section \ref{sec:experiments} and in the Supplementary Material.}
    %
  \item Did you compare performance over time?
    %
    \answerYes{}
    %
  \item Did you perform multiple runs of your experiments and report random seeds?
    %
    \answerYes{We specified the values of the random seeds we used in the Supplementary Material and in the released code.}
    %
  \item Did you report error bars (e.g., with respect to the random seed after
    running experiments multiple times)?
    %
    \answerYes{We provided the standard deviation in the Section \ref{sec:experiments}.}
    %
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    %
    \answerNo{}
    %
  \item Did you include the total amount of compute and the type of resources
    used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    %
    \answerYes{We specified that in the Supplementary Material.}
    %
  \item Did you report how you tuned hyperparameters, and what time and
    resources this required (if they were not automatically tuned by your AutoML
    method, e.g. in a \textsc{nas} approach; and also hyperparameters of your
    own method)?
    %
    \answerYes{We specified that in the Supplementary Material.}
    %
  \end{enumerate}
  %
\item If you are using existing assets (e.g., code, data, models) or
  curating/releasing new assets\dots
  %
  \begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    %
    \answerYes{We cited all the external assets providing either references to the original scientific work or to the url where the source is available.}
    %
  \item Did you mention the license of the assets?
    %
    \answerYes{The used assets were open-source.}
    %
  \item Did you include any new assets either in the supplemental material or as
    a \textsc{url}?
    %
    \answerYes{See the footnote on the second page and Section \ref{sec:experiments}.}
    %
  \item Did you discuss whether and how consent was obtained from people whose
    data you're using/curating?
    %
    \answerNA{}
    %
  \item Did you discuss whether the data you are using/curating contains
    personally identifiable information or offensive content?
    %
    \answerNA{}
    %
  \end{enumerate}
  %
\item If you used crowdsourcing or conducted research with human subjects\dots
  %
  \begin{enumerate}
  \item Did you include the full text of instructions given to participants and
    screenshots, if applicable?
    %
    \answerNA{}
    %
  \item Did you describe any potential participant risks, with links to
    Institutional Review Board (\textsc{irb}) approvals, if applicable?
    %
    \answerNA{}
    %
  \item Did you include the estimated hourly wage paid to participants and the
    total amount spent on participant compensation?
    %
    \answerNA{}
    %
  \end{enumerate}
\end{enumerate}

